Schwinger effect with backreaction in 1+1D massive QED with a strong external field

In the presence of a strong electric field, the vacuum is unstable to the production of pairs of charged particles -- the Schwinger effect. The created pairs extract energy from the electric field, resulting in nontrivial backreaction. In this paper, we study 1+1D massive QED subject to strong external electric fields in a self-consistent and fully quantum manner. We use the bosonized version of the theory, which attains a cosine interaction term in the presence of nonzero fermion mass $m$. However, the assumption of strong electric field justifies a perturbative treatment of the cosine interaction, i.e., an expansion in $m$. We calculate the vacuum expectation value of the electric field to first order in $m$ and show that -- surprisingly -- it satisfies a classical nonlinear partial differential equation (related to the sine-Gordon equation). We show that the electric field exhibits dissipation-free oscillations (analogous to ordinary plasma oscillations) and calculate the plasma frequency analytically. We also compare to the semiclassical approximation commonly used to study backreaction, showing that it fails to capture the $O(m)$ shift in the plasma frequency.

==> Referee_response.tex <==
We thank the referee for their careful reading of the manuscript and for their many constructive and insightful comments. Below, we address each point and indicate the corresponding changes made in the revised version.

1) In the first paragraph of page 8, for example, it is said "q=1, m=0.1, E0=1
(etc)". Units are missing. The plots and the discussion around them (i.e., the
captions) should be in dimensionless quantities, for example m->m/q, E-> E/q and
so on.

We thank the referee for pointing that out. We have revised the manuscript and incorporated the suggested changes. 

2) Gauge invariance and covariance. It would be nice to have a comment [for
example, near eq.(4)] on why the final results are gauge invariant, even if they
used a specific gauge to derive them. Also, would it be possible to write eq.
(4) in a covariant way as well? E is a component of a 2-rank tensor, while \phi
is a (parity odd) scalar.

We thank the referee for the comment. While the derivation was carried out in a specific gauge, our main result yields the expression for the expectation value of the electric field E (Eqs.(3) and (4)). Since E is gauge invariant, our result remains gauge invariant. We have added a comment regarding this point in the text above Eq.(8).

As for the covariance of Eq.(4), it is in the covariant form since in 1+1D, the electric field E behaves as a pseudoscalar. This is because the electric field E is given by  E=F_{10} is invariant under boosts, but parity is odd. We have added a comment below Eq.(29)

3) \theta term. Usually, in the bosonized version of QED_2, there is an extra
(topological) \theta term, which here is fixed to be 0. Can the authors add a
small comment on that?

We thank the referee for raising this point. Within our understanding, the physical interpretation of the theta term is a constant external electric field (for example, Ref. [26]).  In our setup, this corresponds to taking E_C = const. In the present work, we restrict attention to the special case where E_C vanishes at early times in order to define the initial vacuum unambiguously. For this reason, the theta term was taken to be zero. We have added a footnote at the beginning of section III indicating this point. 

If the referee had in mind a different interpretation or role of the theta term—particularly one emphasizing its topological character—we would appreciate any clarification, and we would be happy to address it in a revised version.

4)  \hbar. I understand that the units are such that \hbar=1. However, it would be
nice to comment at some point(s) where \hbar would appear. For example, in (64).
The reason is that the Schwinger rate (e.g., eq. (23) in Ref.
https://arxiv.org/pdf/hep-th/0005078 ) is non-perturbative in \hbar. It will be
interesting to see, based on the results the authors already have, whether the
small m expansion can capture 1/\hbar terms. Without the external field E_C, I
would doubt this is the case (in the same sense that one cannot see a phase
transition using perturbation theory); however, since they include it, it might
be possible to see this effect.

We greatly thank the referee for this helpful comment. In the revised manuscript, we have added Eq. (65) in section IIIC for which \hbar is explicitly restored.  We have also modified the small mass conditions (66) and (67) as well as the following discussion accordingly. The newly added formulas show that the expression is nonanalytic in hbar, indicating that our result is genuinely quantum and cannot be obtained in the limit of hbar->0.  We also emphasize that even when E_C=0, the inverse of \hbar is still present in Eq.(65).   

5) I think calling "fully quantum" to a perturbative approach at leading order is
a bit of an overstatement, since perturbation theory does not capture, in
general, some important effects. If they want to keep it, that's okay; I won't
complain again. However, I think people in general would disagree with that
name.

We thank the referee for this comment. We agree that our analysis is perturbative in the fermion mass and does not capture non-perturbative effects. 
By “fully quantum”, we specifically mean that no expansion in hbar is performed. The newly added formulas and comments in section IIIC would help clarify this.  

6) The addition of the smearing function f(t) around eq. (36) feels a bit
unnatural to me. Could the authors rephrase the explanation a bit? Why isn’t
f(t) in the source term (35)?

We thank the referee for this question. The function f(t) is not intended as a smearing function, but rather as a switching function that turns off the interaction at early times, allowing for a well-defined vacuum state, as explained below Eq. (36). As for Eq.(35), such a function is unnecessary as EC is assumed to be only nonzero after t_0. 


7)  In the section "conservation of energy", they give the result directly and
refer the reader to Appendix B. Although this is a good practice, I would like
them to add at least one more formula. I think the relationship between
\mathcal{E} is related to the Hamiltonian, which deserves one equation.

We thank the referee for this suggestion. We have added Eq. (71) in the main text, explicitly showing that the conserved quantity \mathcal{E} coincides with the expectation value of the Hamiltonian.

8) Typos: between eq. (86) and eq. (87), the sentence "there is not dissipation
AND the order" should read "there is not dissipation AT the order";  In Eq.
(35), you have E(t,x), I guess you mean E_C(t,x); In the 4th line of the second
paragraph of the outlook, the reference to eq. (67) should be in parentheses,
i.e., (67).
We thank the referee for catching these. All listed typos have been corrected in the revised manuscript. 


9) Perturbative vs. saddle point approximations. As discussed above, the authors
compare their approach with the semiclassical approximation [42,43] in the usual
QED_2 setup (without bosonization). This is a good comparison, but I think there
might be a somewhat better comparison. In the bosonized theory, one can also
perform a semiclassical/saddle point approximation, i.e., \phi =\phi_s + \delta
\phi, and study how fluctuations, at leading order, source the equation for
\phi_s. I think Ref. [20] is close to this spirit (even if they do not consider
backreaction).

We thank the referee for the insightful suggestion. Indeed, performing a saddle-point expansion of the bosonized theory is an interesting direction. 
In the massive bosonized theory, however, identifying the appropriate classical equation around which to expand is subtle due to normal ordering ambiguities and the presence of an arbitrary mass scale in the interaction term. One possible systematic approach is the functional renormalization group analysis adopted in Ref. [20]. While very interesting, we believe that a detailed investigation of this comparison goes beyond the scope of the present manuscript.



10) I am unsure whether this is equivalent to the semiclassical approximation in
[42,43] or if it contains additional information. Of course, doing all the
computations is a significant amount of work that goes beyond the scope of this
paper; however, I would appreciate a small comment on this. If the authors plan
to continue with this research line, I do recommend that they take a deeper look
at this comparison. An interesting reference could be:
https://arxiv.org/pdf/hep-th/0304112.
 
Regarding the relation to the semiclassical approximation used in Refs. [42,43], our approach is conceptually different: we neither assume small hbar nor a large N approximation, which is what led to the approximation used in [42,43]. As discussed in Sec. VI, our results show that, in the small-mass limit, effects captured by our calculation are absent in the results of [42,43]. 

We appreciate the referee’s suggestion for the additional reference, and we would be happy to explore this comparison further in future work.

We again thank the referee for their thoughtful comments and helpful suggestions, which have significantly improved the clarity and presentation of the manuscript.


We thank the referee for additional thoughtful comments. Since they did not request any further changes, we did not introduce any additional modifications to the manuscript in response to this comment. Below, we respond to the referee’s comment regarding the subtlety of analyzing the classical limit. 
1) I don’t know if restoring \hbar in the differential equation for <\phi> gives
any extra information about the classical limit, since this limit might depend
on how you define your coupling constants (think about the Klein-Gordon equation
for example). A more appropriate analysis could be, perhaps, to compute the
action S0 (on shell) and compare it with \hbar or to find an essential
singularity in some observable.
We appreciate this comment. In fact, we have been considering the possibility of analyzing the bosonized theory from a classical perspective by starting from the action and taking the hbar -> 0 limit. We will certainly keep these suggestions in mind for future investigations of this question.
We thank the referee again for their helpful remarks and for recommending our paper for publication.


